Analysis and Antenna Position Selection for Pinching-Antenna Systems in Fading Channels

Pinching-antenna systems (PASSs) are an emerging flexible antenna technology that enables the creation of line-of-sight (LoS) links by repositioning a radiating element along a dielectric waveguide (WG). Most existing studies of PASSs assume a purely LoS environment, despite the fact that many practical wireless environments exhibit scattering and spatially correlated shadow fading. In this paper, we present the first statistical analysis of PASS performance under Ricean fading with spatially correlated large-scale fading. Focusing on a fundamental single-user uplink PASS, we characterize the distribution and mean of the maximum achievable signal-to-noise ratio (SNR). For the classical exponentially correlated shadow fading scenario, we express the channel power process in terms of Brownian motion and derive highly accurate approximations for the maximum SNR distribution and mean. For a general class of smoothly correlated shadow fading processes, we derive an accurate expression for the SNR distribution by modeling the process in terms of the fade sojourn duration. To address the challenges of antenna position selection in fading environments, we propose radio environment map (REM)-based positioning strategies, including opportunistic random-look and grid-based constructions. Analytical results are validated by simulation, and the impacts of key system parameters, such as the Ricean $K$-factor, spatial correlation, WG length, and carrier frequency are investigated. The results provide insights into PASS operation beyond idealized LoS conditions and establish a general analytical framework for performance evaluation and antenna positioning in scattered environments.

==> sys_model.tikz.tex <==
\begin{circuitikz}
\tikzstyle{every node}=[font=\LARGE]
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5,14.5) -- (6.25,10);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5,14.5) -- (5,9.75);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5,14.5) -- (3.75,10);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (3.75,10) -- (5.9722,11);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.0278,11) -- (6.25,10);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.0278, 11) -- (5.75, 11.8);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5.75, 11.8) -- (4.42, 12.412);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.25, 11.8) -- (5.58, 12.412);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.25, 11.8) -- (5.9722,11);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.42, 12.412) -- (5.45, 12.8755);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.55, 12.8755) -- (5.58, 12.412);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.55, 12.8755) -- (5.365, 13.2467);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5.45, 12.8755) -- (4.625, 13.2467);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.635, 13.2467) -- (5.295, 13.5504);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.72,13.5504) -- (5.365, 13.2467);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (4.72,13.5504) -- (5.2, 13.7731);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5.28,13.5504) -- (4.8, 13.7731);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5.14,13.9306) -- (4.8, 13.7731);
\draw [line width= 2pt, color={rgb,255:red,14; green,13; blue,99}] (5.2, 13.7731) -- (4.86, 13.9306);

\filldraw [color={rgb,255:red,14; green,13; blue,99}] (5,14.5) circle (5pt);
\draw [ color={rgb,255:red,14; green,13; blue,99}, line width=1pt, short] (6,11) -- (7.25,11);
\draw [ color={rgb,255:red,84; green,122; blue,223} , fill={rgb,255:red,73; green,125; blue,228}, line width=1pt ] (7.25,11.1) rectangle (15.25,10.9);
\draw [ color={rgb,255:red,14; green,13; blue,99} , fill={rgb,255:red,14; green,13; blue,99}, rounded corners = 4.2] (12.1,14.15) rectangle (12.9,12.85);
\draw [ color={rgb,255:red,14; green,13; blue,99} , fill={rgb,255:red,23; green,8; blue,96}, rounded corners = 2] (12.1,14.35) rectangle (12.25,13.75);
\draw [line width=0.5pt, ->, >=Stealth, dashed] (7.25,11) -- (7.25,14.15);
\draw [line width=0.5pt, ->, >=Stealth, dashed] (7.25,11) -- (16.5,11);
\node at (7.25,11) [circ] {};
\draw [ color={rgb,255:red,14; green,13; blue,99} , fill={rgb,255:red,14; green,13; blue,99}] (12.25,11) -- (12.5,10.5) -- (12.75,11) -- (12.5,11.5) -- cycle;
\node [font=\LARGE] at (7.25,14.5) {$y$};
\node [font=\LARGE] at (16.8,11) {$x$};
\node [font=\LARGE] at (7.25,10.25) {$(0,0)$};
\node [font=\LARGE] at (12.5,10) {PA};
\node [font=\LARGE] at (12.5,9.25) {$(x_\mathrm{p}, 0)$};
\node [font=\LARGE] at (7.75,8.25) {};
\node [font=\LARGE] at (5,9.25) {Base Station};
\node [font=\LARGE] at (14.25,13.9) {UE};
\node [font=\LARGE] at (14.25,13.175) {$(x_\mathrm{u}, y_\mathrm{u})$};
\draw [ color={rgb,255:red,14; green,13; blue,99}, line width=1pt, short] (13,11.75) .. controls (12.75,12.2) and (12.25,12.2) .. (12,11.75);
\draw [ color={rgb,255:red,14; green,13; blue,99}, line width=1pt, short] (13.25,11.9) .. controls (13,12.55) and (12,12.55) .. (11.75,11.9);
\draw [ color={rgb,255:red,14; green,13; blue,99}, line width=1pt, short] (12.75,11.6) .. controls (12.75,11.85) and (12.25,11.85) .. (12.25,11.6);
\draw [ color={rgb,255:red,255; green,255; blue,254} , fill={rgb,255:red,255; green,255; blue,254}, rounded corners = 1.2] (12.25,14) rectangle (12.75,13);
\node at (15.25,11) [circ] {};
\node [font=\LARGE] at (15.25,10.25) {$(L,0)$};
\end{circuitikz}
